Randomstrasse101: Open Problems of 2025

Randomstrasse101 is a blog dedicated to Open Problems in Mathematics, with a focus on Probability Theory, Computation, Combinatorics, Statistics, and related topics. This manuscript serves as a stable record of the Open Problems posted in 2025, with the goal of easing academic referencing. The blog can currently be accessed at randomstrasse101.math.ethz.ch

==> figures/5pts_D.tex <==
\begin{tikzpicture}[scale=0.75, outer sep=0]
    % Draw the main filled areas
    \fill[black!40!white] (1, -1) -- (1, -1/3) -- (3, 1) -- (2, 1) -- (2, 2) -- (-1, 2) -- (-1, 1/3) -- (-3, -1) -- cycle;

    % Draw solid lines
    \draw[black!40!white, ultra thick] (1, 2) -- (1, -3);
    \draw[black!40!white, ultra thick] (-1, 1) -- (3, 1);
    \draw[black!40!white, ultra thick] (-1, -1) -- (-1, 2);
    \draw[black!40!white, ultra thick] (1, -1) -- (-3, -1);
    \draw[black!40!white, ultra thick] (-1, 2) -- (2, 2);
    \draw[black!40!white, ultra thick] (2, 1/3) -- (2, 2);

    % New diagonal lines
    \draw[black!40!white, ultra thick] (0, -1) -- (3, 1);
    \draw[black!40!white, ultra thick] (1.5, 2) -- (-3, -1);
    \draw[black!40!white, ultra thick] (2, 2) -- (-2.5, -1);

    % % Draw dotted lines
    % \draw[black, dotted, ultra thick] (1, -1) -- (-3, -1);
    % \draw[black, dotted, ultra thick] (-1, 1) -- (3, 1);
    % \draw[black, dotted, ultra thick] (-1, 2) -- (2, 2);
    % \draw[black, dotted, ultra thick] (-1, 3) -- (-1, -1);
    % \draw[black, dotted, ultra thick] (1, 2) -- (1, -3);
    % \draw[black, dotted, ultra thick] (2, 2) -- (2, 1/3);
    % \draw[black, dotted, ultra thick] (2, 2) -- (-2.5, -1);
    % \draw[black, dotted, ultra thick] (1.5, 2) -- (-3, -1);
    % \draw[black, dotted, ultra thick] (0, -1) -- (3, 1);

    % Draw the points
    \filldraw[black] (3, 1) circle (3pt);
    \filldraw[black] (-1, 2) circle (3pt);
    \filldraw[black] (-3, -1) circle (3pt);
    \filldraw[black] (1, -3) circle (3pt);
    \filldraw[black] (2, 2) circle (3pt);

    % % Add the labels
    % \node at (3.9,1) {$\pi(K_1)$};
    % \node at (0.2,-3) {$\pi(K_2)$}; 
    % \node at (-3.9,-1) {$\pi(K_3)$}; 
    % \node at (-0.2,3) {$\pi(K_4)$}; 
    % \node at (2,2.4) {$\pi(K_5)$};
\end{tikzpicture}
